"Sound and Fury": Nonlinear Functionals of Volatility Matrix in the Presence of Jump and Noise

This paper resolves a pivotal open problem on nonparametric inference for nonlinear functionals of volatility matrix. Multiple prominent statistical tasks can be formulated as functionals of volatility matrix, yet a unified statistical theory of general nonlinear functionals based on noisy data remains challenging and elusive. Nonetheless, this paper shows it can be achieved by combining the strengths of pre-averaging, jump truncation and nonlinearity bias correction. In light of general nonlinearity, bias correction beyond linear approximation becomes necessary. Resultant estimators are nonparametric and robust over a wide spectrum of stochastic models. Moreover, the estimators can be rate-optimal and stable central limit theorems are obtained. The proposed framework lends itself conveniently to uncertainty quantification and permits fully feasible inference. With strong theoretical guarantees, this paper provides an inferential foundation for a wealth of statistical methods for noisy high-frequency data, such as realized principal component analysis, continuous-time linear regression, realized Laplace transform, generalized method of integrated moments and specification tests, hence extends current application scopes to noisy data which is more prevalent in practice.

==> Discussions.tex <==

\subsection{Semi-efficiency}

The efficient bound of volatility estimation is studied by \cite{r11}. Nonetheless, pre-averaging hasn't been able to attain the efficiency bound. According to \cite{jm15}, by taking the moving average adaptively in the time domain, the asymptotic variance of the pre-averaging method can be within 7\% of the efficiency bound. Using adaptive pre-averaging in volatility functional estimation is beyond the scope of this paper and is currently under investigation.

An efficient alternative is the spectral approach \cite{bhmr14, ab15}. The multi-scale approach \cite{zma05}, realized kernels \cite{bhls08}, quasi-likelihood \cite{x10} are equally capable to rate-optimally handle noise. In the univariate case realized kernels and quasi-likelihood could be improved to be nearly efficient, cf. \cite{cp18}. The pre-averaging are adopted in this paper to simultaneously handle price jumps and microstructure noise.
%because a fully extensive study of other estimators is beyond the scope of this paper.
%more essentially due to the limited knowledge of the author.

